Joint Decision-Making in Robot Teleoperation: When are Two Heads Better Than One?

Operators working with robots in safety-critical domains have to make decisions under uncertainty, which remains a challenging problem for a single human operator. An open question is whether two human operators can make better decisions jointly, as compared to a single operator alone. While prior work has shown that two heads are better than one, such studies have been mostly limited to static and passive tasks. We investigate joint decision-making in a dynamic task involving humans teleoperating robots. We conduct a human-subject experiment with $N=100$ participants where each participant performed a navigation task with two mobiles robots in simulation. We find that joint decision-making through confidence sharing improves dyad performance beyond the better-performing individual (p<0.0001). Further, we find that the extent of this benefit is regulated both by the skill level of each individual, as well as how well-calibrated their confidence estimates are. Finally, we present findings on characterising the human-human dyad's confidence calibration based on the individuals constituting the dyad. Our findings demonstrate for the first time that two heads are better than one, even on a spatiotemporal task which includes active operator control of robots.

==> sections/discussion/conclusion.tex <==
\section{CONCLUSION}
We studied human-human dyad joint decision-making on a robot teleoperation task.
We investigated the impact of maximum confidence choice selection on the accuracy of a two-alternative forced-choice task where the objective was to select between two robots, which had different control delays.
We found that the accuracy of the dyad joint decision was significantly higher than the higher performing individual.
The extent of dyadic accuracy gain was regulated by the difference in skill level as well as the difference in confidence calibration between the individuals constituting the dyad.
To the best of our knowledge, this is the first study on joint decision-making for a spatio-temporal dynamic task involving actively controlling robots.
As human-IDS system dyads become increasingly prevalent to enable seamless autonomy, learnings from our study provide interesting directions for future research on joint decision-making for human-IDS system dyads.

==> sections/discussion/future.tex <==

In future work, we plan to build an Intelligent Decision Support (IDS) system for the same task, which will provide decision-making support to human operators selecting between two different robots based on the delay corruption in control.
We will explore both rule-based as well as learning-based approaches to building the IDS system from the gathered human data and investigate further questions in human-IDS system joint decision making for dynamic spatio-temporal tasks.
First, how can we estimate the confidence calibration of the human operator, and how should an IDS system acordingly adapt its confidence calibration so as to enable maximum benefit of MCS for joint decision making?
Second, does human operator confidence calibration change with increased experience on the task, and can that change be influenced by the IDS system?

==> sections/discussion/idsconf.tex <==
These results supplement the existing research on human-IDS joint decision making.
One desideratum for human-IDS pairs is that humans are well calibrated to both their own as well as the IDS decisions~\cite{green2019principles}.
On a collaborative truss design task, it was shown that good human decision makers were those who varied their probability of accepting the IDS recommendation according to their self-confidence and their confidence in the IDS system~\cite{chong2023evolution}.
On a recidivism risk prediction task, it has been shown that humans show well calibrated confidence in their decision making~\cite{aaai2021}.
The role of confidence estimates provided by IDS systems has also been studied in the explanations and trust space.
On a forest cover prediction task, it was found that people use the IDS system's explanation as a proxy for its confidence~\cite{wang2021explanations}.
It was found that confidence estimates provided by IDS systems improved people's trust calibration~\cite{zhang2020effect}.
However, they found that there was no significant benefit to joint decision making when the human operators were provided with IDS system confidence estimates.
We conjecture that this may be because the human operator was still in charge of the final decision and the higher-confidence decision was not taken.

==> sections/discussion/summary.tex <==
The Maximum Confidence Slating approach for joint decision-making showed significantly higher accuracy than the higher performing individual.
% We established a principled way to select between choices made by a dyad of human operators on our robot selection task: select the choice made with higher confidence.
To the best of our knowledge, this is the first study investigating the impact of MCS on a task where humans have to actively control robots as compared to passively receiving information.

The effect of MCS was governed by the difference in both the skill as well as confidence calibration of the individuals constituting the dyads. 
We found that pairing participants of similar skill level led to a higher accuracy gain as compared to pairing participants of dissimilar skill.
Similar results have also been reported in the literature where pairing participants of similar visual senstivity led to the benefit of MCS being observed~\cite{bahrami2010optimally}.

% How well the two individuals' confidence was calibrated has a significant impact on the benefit of maximum confidence selection.
% Metacognitive “sensitivity” is defined as the trial-by-trial relationship between confidence and performance. 
% In a person with high levels of metacognitive sensitivity, trials with high confidence would be very likely to be correct trials, while trials with low confidence would be at chance levels of performance. 
% This person’s confidence would closely track their accuracy, on a trial-by-trial basis. 
% In contrast, a person with very low levels of metacognitive sensitivity would be no more likely to be correct on trials when their confidence judgements were high than those when their confidence judgements were low~\cite{fleming2014measure}.

Further, pairing participants according to how well their confidence was calibrated also impacted the benefit obtained by MCS on the dyad.
When both participants were well calibrated, the higher confidence joint decision was more accurate.
Further, the accuracy gain (difference in percentage accuracy of higher confidence choice versus choice made by more performant individual) obtained was correlated with the dyadic confidence calibration: an increase in dyadic confidence calibration led to an increased gain in accuracy.
On the other hand, we found that using MCS when both participants had poor confidence calibration was detrimental to joint decision-making.
% These results add to the existing literature on the benefit of MCS on joint decision making.
% While prior studies found that participants needed to be of similar skill level (for example, visual sensitivity~\cite{bahrami2010optimally}) for MCS to provide a team benefit, we found that confidence calibration of the individuals also has a significant impact.

% \textcolor{blue}{We also found that confidence calibration of individuals impacts dyad confidence calibration. And dyad confidence calibration impacts 2habt1.}



==> sections/experiment/traces.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width= \textwidth]{sections/figures/traces2.png}
%     \caption{Paths followed by various participants starting from two different initial locations. Each color represents the path driven by a different participant, showcasing the variability in their manueuvers.}
%     \label{fig:traces}
% \end{figure*}

==> sections/hypotheses/hypotheses.tex <==
\section{HYPOTHESES}

Building on the body of related work described above, we thus formulate two key research questions:
\begin{itemize}
    \item[] \textbf{RQ1:} Can a virtual robotic arm perform tasks as accurately and as efficiently as a physical robot arm while offering users a similarly natural interaction?
    \item[] \textbf{RQ2:} When there is a mismatch between the reality of the robot arm and the referent, will accuracy, efficiency, and subjective perception be affected?
\end{itemize}
Our work accordingly seeks to assess two sets of hypotheses.

==> sections/relatedwork/dss.tex <==
AI-driven decision aids are being used in recidivism risk prediction~\cite{dss_whentoadvice,chiang2023two}, content moderation~\cite{keswani2021towards}, medical diagnosis~\cite{multiplehumans_ijcai22} and rental price bidding~\cite{wang2023effects}.
The operation of decision aids with a team of two or more human operators has also been studied recently.
Algorithms have been proposed for the decision aid to optimally defer to one out of multiple possible human experts~\cite{keswani2021towards,multiplehumans_ijcai22}.
Whether two humans with a decision aid are better than one human with a decision aid has also been investigated~\cite{chiang2023two}.
Most of these decision aids are deployed in a setup with human-initiative control~\cite{chiou2021mixed}, where the final decision to accept or reject the recommendation lies with the human operator.
Research is needed to determine how best to deploy these systems as a joint decision maker with a human operator.

==> sections/relatedwork/idsconf.tex <==
The use of confidence estimates in IDS systems has also been studied.
Recent examples include confidence estimates associated with choices in an income class prediction task~\cite{zhang2020effect}, with recidivism risk prediction on a classifier trained on the COMPAS dataset~\cite{grgic2019human}, and less certain tokens on a neural machine translation task~\cite{weisz2021perfection}.


==> sections/relatedwork/idsrobots.tex <==
Robots have strong potential as decision-support systems in human-robot teams. 
While AI-driven decision support systems are established across numerous industries, only recently has the human-robot interaction
(HRI) community applied robots as decision-support in real world applications.
In human-robot teaming domains, robot partners can use their understanding of the world state and other teammates to present recommendations on taskwork division, team strategy, and world state interpretation.
Researchers have sought to provide robots with an active role in team decision-making across domains including space operation for location marking~\cite{gervits2020toward}, command of UAV swarm for bushfire search~\cite{lim2021adaptive}, emergency evacuation~\cite{robinette2016overtrust}, and collaborative construction~\cite{idsrobot_construction}.

==> sections/relatedwork/metacog.tex <==
The importance of confidence estimation in joint decision-making suggests a key role for metacognition~\cite{dunlosky2008metacognition}, the ability to assess one's own task performance.
Accurate metacognition is thought to optimise learning strategies, for instance, in education by contributing to efficient cognitive offloading, or protecting against cognitive biases~\cite{fleming2021know}. 
Therefore, understanding the role of metacognition is a key goal for decision-making in human-robot collaboration.
The fidelity of metacognition is typically assessed by asking how subjective judgements - such as confidence - track objective performance. 
Metacognitive “sensitivity” is defined as the trial-by-trial relationship between confidence and performance. 
In a person with high levels of metacognitive sensitivity, trials with high confidence would be very likely to be correct trials, while trials with low confidence would be at chance levels of performance. 
This person’s confidence would closely track their accuracy, on a trial-by-trial basis. 
In contrast, a person with very low levels of metacognitive sensitivity would be no more likely to be correct on trials when their confidence judgements were high than those when their confidence judgements were low~\cite{fleming2014measure}.

==> sections/results/figs/conf-hist.tex <==

Figure~\ref{fig:conf-histogram} shows the histogram of confidence values over all the participants over all trials. 
The percentage of participant responses with Lowest Confidence is 15.8\%, Low Confidence is 28.2\%, High Confidence is 30.1\%, and Highest Confidence is 25.9\%.


